Offline Policy Optimization in RL with Variance Regularizaton

Learning policies from fixed offline datasets is a key challenge to scale up reinforcement learning (RL) algorithms towards practical applications. This is often because off-policy RL algorithms suffer from distributional shift, due to mismatch between dataset and the target policy, leading to high variance and over-estimation of value functions. In this work, we propose variance regularization for offline RL algorithms, using stationary distribution corrections. We show that by using Fenchel duality, we can avoid double sampling issues for computing the gradient of the variance regularizer. The proposed algorithm for offline variance regularization (OVAR) can be used to augment any existing offline policy optimization algorithms. We show that the regularizer leads to a lower bound to the offline policy optimization objective, which can help avoid over-estimation errors, and explains the benefits of our approach across a range of continuous control domains when compared to existing state-of-the-art algorithms.

==> 10_broader_impacts.tex <==
\newpage
\section*{Broader Impact}
Our work relates to batch offline reinforcement learning, which is crucial for scaling up RL algorithms for practical applications, espeically in healthcare domains or marketing applications. In healthcare systems, often data is expensive to collect, and requires full utilization of available data. Batch offline RL provides a way towards this, especially when solving the task requires sequential decision making under fixed data. Furthermore, our work also relates to risk-sensitive optimization and safe RL, which has a number of applications beyond academia. For example, in robotic systems and autonomous driving,  it is imperative to prevent collisions of the car with objects/people on the road even during training. Similarly, in manipulation tasks, we want to ensure that the work space is not damaged by a robotic arm and in turn the arms do not get damaged by rigid objects it interact with. Learning RL policies under constraints, ensuring safety when deploying the agent for real world applications is therefore of vital importance for success of artificial general systems to be useful for the society.



% Our work relates to risk-sensitive optimization and safe reinforcement learning which has a number of implications beyond academia.
% For example, in real robotic systems like autonomous driving, it is imperative to prevent collisions of the car with objects/people on the road even during training.
% Similarly, in manipulation tasks, we want to ensure that the workspace is not damaged by a robotic arm and in turn the end effectors of the arm do not get damaged by rigid objects it interact with. Hence, safety is of practical interest while deploying autonomous systems in the real world as unsafe actions can be costly for robots as well as the equipment.
% \Sam{i wouldnt add this} Although we do not provide any probabilistic safety guarantees through constraint satisfaction in this work, and make no guarantees about the safety of the policy used to collect the offline dataset, our work ... We intend to explore safety more rigorously in future work. 
